An hp-hierarchical framework for the finite element exterior calculus

The problem of solving partial differential equations (PDEs) on manifolds can be considered to be one of the most general problem formulations encountered in computational multi-physics. The required covariant forms of balance laws as well as the corresponding covariant forms of the constitutive closing relations are naturally expressed using the bundle-valued exterior calculus of differential forms or related algebraic concepts. It can be argued that the appropriate solution method to such PDE problems is given by the finite element exterior calculus (FEEC). The aim of this essay is the exposition of a simple, efficiently-implementable framework for general hp-adaptivity applicable to the FEEC on higher-dimensional manifolds. A problem-independent spectral error-indicator is developed which estimates the error and the spectral decay of polynomial coefficients. The spectral decay rate is taken as an admissibility indicator on the polynomial order distribution. Finally, by elementary computational examples, it is attempted to demonstrate the power of the method as an engineering tool.

==> figures/elasticity.tex <==
%!TEX root = ../nmedoc.tex
\begin{minipage}{0.45\textwidth}
\begin{center}
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
	\includegraphics[width=.8\textwidth]{./figures/images/elasticity/res/cut/screenshot_67-sol2}
      };
      \node (label) at (0.05,-4.0)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = BuRd,
    colorbar horizontal,
    point meta min=-3.088e-2,
    point meta max=7.771,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-1.5cm,
        height=.25cm,
        }
        ]};
      \draw[-stealth, thick] (-2,-2.5)--(-2,-1.5) node[above] {$x_2$};  
      \draw[-stealth, thick] (-2,-2.5)--(-1,-2.5) node[right] {$x_1$};  
\end{tikzpicture}\\
(a) Vertical displacement
\vspace{.25cm}
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
\includegraphics[width=\textwidth]{./figures/images/elasticity/res/rot/cut/elast_1}
      };
      \node (label) at (0.05,-3.9)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = arnold,
    colorbar horizontal,
    point meta min=-519.1,
    point meta max=13.84,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-1.5cm,
        height=.25cm,
        }
        ]};
%      \draw[-stealth, thick] (2.25,-1.5)--(1.65,-1.25) node[above] {$-x_1$};  
%      \draw[-stealth, thick] (2.25,-1.5)--(2.25,-2.25) node[left] {$-x_2$};  
%            \draw[-stealth, thick] (2.25,-1.5)--(2.75,-1.35) node[above] {$-x_3$};  
\draw[-stealth, thick] (2.25,-1.5)--(2.95,-1.7) node[right] {$x_1$};  
      \draw[-stealth, thick] (2.25,-1.5)--(2.17,-0.75) node[above] {$x_2$};  
            \draw[-stealth, thick] (2.25,-1.5)--(1.65,-1.65) node[below] {$x_3$};  
\end{tikzpicture}\\
(c) Hydrostatic stress $\frac{1}{3}\mrm{tr}(\star_{\bs{g}}\mbb{t})$ 
\end{center}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\centering
\begin{center}
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
\includegraphics[width=.8\textwidth]{./figures/images/elasticity/res/cut/screenshot_67-err_f2}
      };
      \node (label) at (0.05,-4.0)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = arnold,
    colorbar horizontal,
    point meta min=-0,
    point meta max=1.693,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-1.5cm,
        height=.25cm,
        }
        ]};
     \draw[-stealth, thick] (-2,-2.5)--(-2,-1.5) node[above] {$x_2$};  
      \draw[-stealth, thick] (-2,-2.5)--(-1,-2.5) node[right] {$x_1$};  
\end{tikzpicture}\\
(b) Relative error
\vspace{.25cm}
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
\includegraphics[width=\textwidth]{./figures/images/elasticity/res/rot/cut/elast_2}
      };
      \node (label) at (0.05,-3.9)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = arnold,
    colorbar horizontal,
    point meta min=1,
    point meta max=8,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-1.5cm,
        height=.25cm,
        }
        ]};
      \draw[-stealth, thick] (2.25,-1.5)--(2.95,-1.7) node[right] {$x_1$};  
      \draw[-stealth, thick] (2.25,-1.5)--(2.17,-0.75) node[above] {$x_2$};  
          %  \draw[-stealth, thick] (2.25,-1.5)--(1.75,-1.7) node[left] {$x_3$};  
\end{tikzpicture}\\
(d) Hierarchical subdivision depth
\end{center}
\end{minipage}

==> figures/geometric_decomposition.tex <==
%!TEX root = ../nmedoc.tex
\newcommand\IMAGESWIDTHBD{.22}

\begin{figure}[htb]
	\centering
	\begin{minipage}[t]{\IMAGESWIDTHBD\linewidth}
        		\begin{tikzpicture}
			\node[inner sep=0pt]{\includegraphics[trim={35cm 20cm 37cm 14cm},clip,width=\linewidth]{./figures/images/vertices_dim_2.png}};
			\node at (-.92,-.8) {$f_{(1)}$};
			\node at (1.17,-.8) {$f_{(2)}$};
			\node at (.5,.8) {$f_{(3)}$};
		\end{tikzpicture}
		\begin{center}
        		(a) $\Dksimplx{T}{0}$
		\end{center}
    	\end{minipage}% <- sonst wird hier ein Leerzeichen eingefügt
    	\hfill
    	\begin{minipage}[t]{\IMAGESWIDTHBD\linewidth}
		\begin{tikzpicture}
			\node[inner sep=0pt]{\includegraphics[trim={35cm 20cm 37cm 14cm},clip,width=\linewidth]{./figures/images/lines_dim_2.png}};
			\node at (-1.,.2) {$f_{(1,3)}$};
			\node at (0.2,-0.65) {$f_{(1,2)}$};
			\node at (1.3,.2) {$f_{(2,3)}$};
		\end{tikzpicture}
        		\begin{center}
        		(b) $\Dksimplx{T}{1}$		
		\end{center}
	\end{minipage}%
	\hfill
    	\begin{minipage}[t]{\IMAGESWIDTHBD\linewidth}
		\begin{tikzpicture}
			\node[inner sep=0pt]{\includegraphics[trim={35cm 20cm 37cm 14cm},clip,width=\linewidth]{./figures/images/face_dim_2.png}};
			\node at (0.15,-0.3) {$f_{(1,2,3)}$};
		\end{tikzpicture}
        		\begin{center}
        		(c) $\Dksimplx{T}{2}$
		\end{center}
	\end{minipage}%
	\hfill
    	\begin{minipage}[t]{\IMAGESWIDTHBD\linewidth}
		\begin{tikzpicture}
			\node[inner sep=0pt]{\includegraphics[trim={35cm 20cm 37cm 14cm},clip,width=\linewidth]{./figures/images/cl_T_dim_2.png}};
		\end{tikzpicture}
        		\begin{center}
        		(d) $\simplx{T} = \mrm{cl}(f_{(1,2,3)})$
		\end{center}
	\end{minipage}%
	\caption{Geometric decomposition of 2-simplex}
\end{figure}




==> figures/incomplete_freudenthal.tex <==
%!TEX root = ../nmedoc.tex
\newcommand\IMAGESWIDTHIF{.3}

\begin{figure}[htb]
	\centering
	\begin{minipage}[t]{\IMAGESWIDTHIF\linewidth}
        		\begin{tikzpicture}
			\node[inner sep=0pt]{\includegraphics[trim={29cm 11cm 30cm 3cm},clip,width=\linewidth]{./figures/images/level1_simplex_dim_3.png}};
	 	\node at (0.025,-1.75) {$v_{1}$};
		\node at (2.3,-1.75) {$v_{2}$};
		\node at (-2.1,-1.7) {$v_{3}$};
		\node at (0.0,2.025) {$v_{4}$};
		\end{tikzpicture}
		\begin{center}
        		(a) unrefined subsimplices $\Dsimplx{T}$
		\end{center}
    	\end{minipage}% <- sonst wird hier ein Leerzeichen eingefügt
    	\hfill
    	\begin{minipage}[t]{\IMAGESWIDTHIF\linewidth}
		\begin{tikzpicture}
			\node[inner sep=0pt]{\includegraphics[trim={29cm 11cm 30cm 3cm},clip,width=\linewidth]{./figures/images/red_refinement_dim_3.png}};
		\end{tikzpicture}
        		\begin{center}
        		(b) complete Freudenthal $\Dkfreud{\simplx{T}}{}$
		\end{center}
	\end{minipage}%
	\hfill
    	\begin{minipage}[t]{\IMAGESWIDTHIF\linewidth}
		\begin{tikzpicture}
			\node[inner sep=0pt]{\includegraphics[trim={29cm 11cm 30cm 1cm},clip,width=\linewidth]{./figures/images/vertex_refinement_dim_3.png}};
		\end{tikzpicture}
        		\begin{center}
        		(c) vertex refinement $\incfreud{\simplx{T},f_{(1)}}$
		\end{center}
	\end{minipage}%
	\hfill
    	\begin{minipage}[t]{\IMAGESWIDTHIF\linewidth}
		\begin{tikzpicture}
			\node[inner sep=0pt]{\includegraphics[trim={29cm 11cm 30cm 1cm},clip,width=\linewidth]{./figures/images/line_refinement_dim_3.png}};
		\end{tikzpicture}
        		\begin{center}
        		(d) line refinement $\incfreud{\simplx{T},f_{(1,2)}}$
		\end{center}
	\end{minipage}%
	\hfill
    	\begin{minipage}[t]{\IMAGESWIDTHIF\linewidth}
		\begin{tikzpicture}
			\node[inner sep=0pt]{\includegraphics[trim={29cm 11cm 30cm 1cm},clip,width=\linewidth]{./figures/images/face_refinement_dim_3.png}};
		\end{tikzpicture}
        		\begin{center}
        		(e) face refinement $\incfreud{\simplx{T},f_{(1,2,4)}}$
		\end{center}
	\end{minipage}%
	\hfill
    	\begin{minipage}[t]{\IMAGESWIDTHIF\linewidth}
		\begin{tikzpicture}
			\node[inner sep=0pt]{\includegraphics[trim={29cm 11cm 30cm 1cm},clip,width=\linewidth]{./figures/images/volume_refinement_dim_3.png}};
		\end{tikzpicture}
        		\begin{center}
        		(f) volume refinement $\incfreud{\simplx{T},f_{(1,2,3,4)}}$
		\end{center}
	\end{minipage}%
	\caption{Leaf vertices, edges and faces of the incomplete Freudenthal subdivision of a tetrahedron $\protect\simplx{T}$. The volumes are omitted in the graphics. They exist on the root level in (a) as well as on the refined level in the remaining depictions.}
\end{figure}




==> figures/lshape_error_decay_rate.tex <==
%!TEX root = ../nmedoc.tex
\begin{minipage}{0.3\textwidth}
\centering
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
	\includegraphics[width=\textwidth]{./figures/images/hodgelaplacian/2D/K2/res/screenshot_1-err_f1.png}
      };
      \node (label) at (0,-2.8)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = arnold,
    colorbar horizontal,
    point meta min=0.0,
    point meta max=611.7,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-.5cm,
        height=.25cm,
        }
        ]};
\end{tikzpicture}\\
(a) Relative error for $\bs{\sigma} \in {\Lambda^1}$
%\caption*{Polynomial order distribution}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
\centering
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
	\includegraphics[width=\textwidth]{./figures/images/hodgelaplacian/2D/K2/res/screenshot_1-err_fs.png}
      };
      \node (label) at (0,-2.8)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = arnold,
    colorbar horizontal,
    point meta min=-3.060e-1,
    point meta max=2.152e2,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-.5cm,
        height=.25cm,
        }
        ]};
\end{tikzpicture}\\
(b) Relative error for $\bs{u} \in {\Lambda^2}$
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
\centering
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
	\includegraphics[width=\textwidth]{./figures/images/hodgelaplacian/2D/K2/res/screenshot_1-err_dec_rate.png}
      };
      \node (label) at (0,-2.8)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = arnold,
    colorbar horizontal,
    point meta min=2.24e-1,
    point meta max=3,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-.5cm,
        height=.25cm,
        }
        ]};
\end{tikzpicture}\\
   %\includegraphics[width=\textwidth]{./figures/images/hodgelaplacian/2D/K2/res/screenshot_1-err_dec_rate.png}
(c) Cumulative decay rate
\end{minipage}


==> figures/lshape_solution_u.tex <==
%!TEX root = ../nmedoc.tex
\begin{minipage}{0.49\textwidth}

\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
	\includegraphics[width=\textwidth]{./figures/images/hodgelaplacian/2D/K2/res/screenshot_1-sol2.png}
      };
      \node (label) at (0,-2.5)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = BuRd,
    colorbar horizontal,
    point meta min=-4.058e-3,
    point meta max=0.5049,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-1.5cm,
        height=.25cm,
        }
        ]};
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
	\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
	\includegraphics[width=\textwidth]{./figures/images/hodgelaplacian/2D/K2/res/screenshot_69-sol2.png}
      };
      \node (label) at (0,-2.5)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = BuRd,
    colorbar horizontal,
    point meta min=-4.056e-5,
    point meta max=0.4682,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-1.5cm,
        height=.25cm,
        }
        ]};
\end{tikzpicture}
\end{minipage}

==> figures/refined_laplacian_2d_k2.tex <==
%!TEX root = ../nmedoc.tex
\begin{minipage}{0.45\textwidth}
\centering
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
	\includegraphics[width=\textwidth]{./figures/images/hodgelaplacian/2D/K2/res/screenshot_69-wireframe.png}
      };
      \node (label) at (0,-4.0)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = BkOr,
    colorbar horizontal,
    point meta min=1,
    point meta max=6,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-.5cm,
        height=.25cm,
        }
        ]};
\end{tikzpicture}\\
(a) Hierarchical subdivision depth
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\centering
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
\includegraphics[width=\textwidth]{./figures/images/hodgelaplacian/2D/K2/res/screenshot_69-err_fs.png}
      };
      \node (label) at (0,-4.0)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = arnold,
    colorbar horizontal,
    point meta min=0.0,
    point meta max=1.659,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-.5cm,
        height=.25cm,
        }
        ]};
\end{tikzpicture}\\
(b) Relative error for $\bs{u} \in \mc{P}^-\Lambda^2$
\end{minipage}\vspace{.3cm}\\
\begin{minipage}{0.45\textwidth}
\centering
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
\includegraphics[width=\textwidth]{./figures/images/hodgelaplacian/2D/K2/res/screenshot_69-err_dec_rate.png}
      };
      \node (label) at (0,-4.0)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = arnold,
    colorbar horizontal,
    point meta min=0.5278,
    point meta max=5,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-.5cm,
        height=.25cm,
        }
        ]};
\end{tikzpicture}\\
(c) Cumulative decay rate
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\centering
\begin{tikzpicture}[every node/.style={inner sep=2,outer sep=0}]
\node (label) at (0,0)[]{
\includegraphics[width=\textwidth]{./figures/images/hodgelaplacian/2D/K2/res/screenshot_69-p_order.png}
      };
      \node (label) at (0,-4.0)[  ]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = Purples,
    colorbar horizontal,
    point meta min=1,
    point meta max=7,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
        width=\textwidth-.5cm,
        height=.25cm,
        }
        ]};
\end{tikzpicture}\\
(d) Polynomial order distribution
\end{minipage}


==> figures/zoom.tex <==
%!TEX root = ../nmedoc.tex
\begin{center}
\begin{tikzpicture}
\node[inner sep=0pt] (sc1) at (-3.5,0)
    {\includegraphics[height=5.5cm]{./figures/images/elasticity/p_order_scale_1}};
\node[draw,rectangle,inner sep=0pt,line width=2] (sc2) at (1.,0)
    {\includegraphics[height=4cm]{./figures/images/elasticity/p_order_scale_2}};
    \node[draw,rectangle,inner sep=0pt,line width=2] (sc3) at (4.85,0)
    {\includegraphics[height=4cm]{./figures/images/elasticity/p_order_scale_3}};
      %  \node[inner sep=0pt] (sc3) at (0,-3.5)
   % {\includegraphics[width=.5\textwidth]{./figures/images/elasticity/p_order_scale_colorbar}};
	\node[draw,rectangle,minimum height=.8cm,minimum width=.8cm,line width=1] (scb1) at (-1.65,-2.35){};
	\draw[-stealth,line width = 1] (scb1) --  (-0.25,-1.5);	
	\node[draw,rectangle,minimum height=1.25cm,minimum width=1.0cm,line width=1] (scb2) at (2.325,-1.325){};
	\draw[-stealth,line width = 1] (scb2) --  (3.75,-1.25);
	  \node (label) at (.35,-3.5)[]{
\pgfplotscolorbardrawstandalone[ 
    colormap name = arnold,
    colorbar horizontal,
    point meta min=1,
    point meta max=7,
    colorbar style={
	%yticklabel={\footnotesize \pgfmathparse{10^\tick}\pgfmathprintnumber\pgfmathresult},
    	%scaled ticks=false,
	xtick={1,2,...,7},
        height=.25cm,
        width=5cm,
        }
        ]};	
\end{tikzpicture}
\end{center}

